Estimation of Shortest Path Covariance Matrices

We study the sample complexity of estimating the covariance matrix $\mathbf{\Sigma} \in \mathbb{R}^{d\times d}$ of a distribution $\mathcal D$ over $\mathbb{R}^d$ given independent samples, under the assumption that $\mathbf{\Sigma}$ is graph-structured. In particular, we focus on shortest path covariance matrices, where the covariance between any two measurements is determined by the shortest path distance in an underlying graph with $d$ nodes. Such matrices generalize Toeplitz and circulant covariance matrices and are widely applied in signal processing applications, where the covariance between two measurements depends on the (shortest path) distance between them in time or space. We focus on minimizing both the vector sample complexity: the number of samples drawn from $\mathcal{D}$ and the entry sample complexity: the number of entries read in each sample. The entry sample complexity corresponds to measurement equipment costs in signal processing applications. We give a very simple algorithm for estimating $\mathbf{\Sigma}$ up to spectral norm error $\epsilon \left\|\mathbf{\Sigma}\right\|_2$ using just $O(\sqrt{D})$ entry sample complexity and $\tilde O(r^2/\epsilon^2)$ vector sample complexity, where $D$ is the diameter of the underlying graph and $r \le d$ is the rank of $\mathbf{\Sigma}$. Our method is based on extending the widely applied idea of sparse rulers for Toeplitz covariance estimation to the graph setting. In the special case when $\mathbf{\Sigma}$ is a low-rank Toeplitz matrix, our result matches the state-of-the-art, with a far simpler proof. We also give an information theoretic lower bound matching our upper bound up to a factor $D$ and discuss some directions towards closing this gap.

==> append.tex <==
% !TEX root = main.tex

\section{Appendix}
In \cite{toep}, the author established the bounds for the Toeplitz structured covariance matrix. In the context of this paper, the underlying graph structure of the Toeplitz matrix is a chain graph with $d$ nodes. So the diameter of the graph is $D=d-1$ and we can apply a sparse ruler of $\Theta(\sqrt{d})$ along with Algorithm~\ref{alg:est} to estimate the covariance. In the proof of Theorem 4.3 of \cite{toep}, the authors provided a sample complexity proof with the help of Vandermonde decomposition \cite{pisarenko1973retrieval} of Toeplitz matrix and  \emph{discrete time Fourier Transform}. Here we provide a simpler  technique where we use a mathematical tool called 'circulant embedding' and use the Fourier structure of the circulant matrix to proof the sample complexity.



\subsection{Circulant Matrix}
A $d\times d$ circulant matrix takes the form
\[ \mathbf{C}=
\begin{bmatrix}
    c_{0}  & c_{d-1} & c_{d-2} & \dots & c_{2} & c_{1} \\
    c_{1}   & c_{0}  & c_{d-1} & \dots & c_{3} & c_{2} \\
    \hdotsfor{5} \\
    c_{d-1} & c_{d-2} & c_{d-3} & \dots & c_{1} & c_{0}
\end{bmatrix}
\]\\
So the matrix can be expressed using permutation of the first column $\mathbf{c}=(c_0,c_1,\ldots,c_{d-1}) $. Also circulant matrix have the following nice property 
\begin{align}
    \mathbf{C}= \mathbf{F}\mathbf{\Lambda}\mathbf{F}^* \label{dft}
\end{align}
where $\mathbf{F}$ is $d\times d$ DFT matrix and $\mathbf{\Lambda} =diag(F\mathbf{c})=diag(c(\omega_0),c(\omega_1),\ldots ,c(\omega_{d-1}))$. $c(x)$ is a polynomial with the co-efficient of the entries of the vector $\mathbf{c}$.
\begin{align}
    c(x)=\mathbf{c}_0+\mathbf{c}_1x+ \ldots + \mathbf{c}_{d-1}x^{d-1} \label{poly}
\end{align}
Now we can bound the $\ell_2 $ norm of the matrix as follows \cite{lindner2018circulant}
\begin{align*}
   \left\| \mathbf{C} \right\|= \left\|\mathbf{F}\mathbf{\Lambda}\mathbf{F}^* \right\| =\left\|\mathbf{\Lambda}\right\|=\max_{j}\left\|c(\omega_j)\right\|
\end{align*}
where $\omega_j=\exp(\frac{2\pi}{d}\mathbf{i}) ; (\mathbf{i}=\sqrt{-1})$.


Given a Toeplitz matrix $\mathbf{T}$ that is described by $(2d-1)$ entries
$\{t_0,t_{-1},\ldots t_{-d+1},t_1,\ldots t_{d-1}\}$. For a symmetric toeplitz we have $t_i=t_{-i}$. Now we can embed the matrix in a $2d\times 2d$  circulant matrix $\mathbf{C}_{\mathbf{T}}$ with element in the first row $\{t_0, t_1,\ldots t_{d-1},0,t_{d-1},t_{d-2},\ldots t_1\}$. The norm of the Toeplitz matrix can be bounded as follows with circulant embedding and Equation~\eqref{poly},~\eqref{dft}
\begin{align*}
 \left\|\mathbf{T}\right\| & \leq  \left\|\mathbf{C}_{\mathbf{T}}\right\| \\
 & =\max_{k\in \{0,1\ldots 2d-1\}}t_0+ 2\sum_{j=1}^{d-1}t_jcos(jk\frac{2\pi}{2d}\textbf{i})
\end{align*}
 We make use of the following well known concentration inequality.
 \begin{lemma}[Henson-Wright Inequality]\cite{rudelson2013hanson}\label{lem:hens}
 Let $\x^{1},\ldots,x^{n} \sim \mathcal{N}(0,\mathbf{I})$ be independent. There exists a universal constant $c>0$ so that for all $\mathbf{A}\in \mathbb{R}^{d\times d}$ and all $t>0$,
 \begin{align*}
     Pr\left[ \left|\frac{1}{n}\sum_{l=1}^n \x^{l^T}\mathbf{A}\x^{l}-Tr(\mathbf{A})  \right|>t  \right] \leq 2\exp \left( -c\,n \min \left( \frac{t^2}{\left\|\mathbf{A} \right\|_F^2 } ,\frac{t}{\left\|\mathbf{A} \right\|_2 }\right)\right).
 \end{align*}
 
 \end{lemma}


\begin{theorem}\label{thm:toep}
For any positive semidefinite Toeplitz covariance matrix $\bSigma \in \mathbb{R}^{d \times d}$, Algorithm ~\ref{alg:est} returns $\Tilde{\bSigma} $ such that $\|\bSigma- \Tilde{\bSigma}\|_2 \leq \epsilon\|\Tilde{\bSigma}\|_2 $ with entry sample complexity $\theta(\sqrt{d})$ and vector sample complexity $n= \frac{1}{c\kappa}\log (\frac{d}{\delta})$ with probability $1-\delta $ for any $\epsilon,\delta>0$, where $\kappa = \min(1, \frac{\epsilon^2\|\bSigma\|_2^2}{\Delta(R)\|\bSigma_R\|_2^2})$.
\end{theorem}

\begin{proof}
Say $\Tilde{\bSigma}$ is the output co-variance matrix according to the  Algorithm~\ref{alg:est}. We assume that the matrix $\bSigma$ is a symmetric Toeplitz matrix. So the error $\bSigma-\Tilde{\bSigma} $ is also a symmetric Toeplitz matrix. Say $\mathbf{e}$ is the associated vector to the error matrix(Toeplitz). Now form the circulant embedding argument we can state that 
\begin{align*}
   \left \|\bSigma-\Tilde{\bSigma}\right\|_2 &\leq \max_{k\in \{0,1\ldots 2d-1\}}\mathbf{e}_0+ 2\sum_{j=1}^{d-1}\mathbf{e}_jcos(jk\frac{2\pi}{2d})\\
    & = \max_{k\in \{0,1\ldots 2d-1\}}\mathbf{e}_0+ 2\sum_{j=1}^{d-1}\mathbf{e}_jcos(2\pi j x)\\
    &= \max_{x }  L_e(x)
\end{align*}

where $x= \frac{k}{2d} \quad  k= \{ 0,1\ldots ,2d-1\}$ .

We define the error vector $\mathbf{e}$ in the following manner. For $s \in . \{0,\ldots d-1\}$
\begin{align*}
    \mathbf{e}_s= \frac{1}{n|R_s|} \sum_{l=1}^n \sum_{(j,k)\in R_s}\left[\bSigma_{j,k}- \x^{(l)}_j\x^{(l)}_k \right]
\end{align*}
Now fix one value of $x$ 
\begin{align*}
    L_{e}(x) &= \sum_{s=0}^{d-1}\left[\frac{1}{n|R_s|} \sum_{l=1}^n \sum_{(j,k)\in [d] : |j-k|=s}\left[\bSigma_{j,k}- \x^{(l)}_j\x^{(l)}_k \right] \right]cos(2\pi s x) \\
    & =\sum_{s=0}^{d-1} \sum_{(j,k)\in [d] : |j-k|=s}\left[\bSigma_{j,k}- \frac{1}{n}\sum_{l=1}^n\x^{(l)}_j\x^{(l)}_k \right]\frac{cos(2\pi s x)}{|R_s|}\\
    & =Tr\left(\bSigma_R-\Bar{\bSigma}_R,\mathbf{M}_R \right) 
\end{align*}

The subscript $R$ denotes the sub-matrix indexed by the ruler. Now assume that $\x_R^{(l)}$ denotes the sample restricted to the ruler. So we have $\x_R^{(l)} \sim \mathcal{N}(0,\bSigma_R)$. If we let $\y^{(l)}=\bSigma_R^{-1/2}\x^{(l)}_R$ then $\y^{(l)}$ is a standard normal vector. Now we have
\begin{align*}T^
    Tr\left(\bSigma_R-\Bar{\bSigma}_R,\mathbf{M}_R \right)& = Tr\left(\bSigma_R,\mathbf{M}_R \right)-\frac{1}{n}\sum_{l=1}^m {\x_R^{(l)}}^T \mathbf{M}_R \x_R^{(l)}\\
    & = Tr(\mathbf{M}'_R)- \frac{1}{n}\sum_{l=1}^m {\y^{(l)}}^T \mathbf{M}'_R \y^{(l)}
\end{align*}
 where $\mathbf{M}'_R=\bSigma_R^{1/2}\mathbf{M}_R\bSigma_R^{1/2}$. Observe that
\begin{align*}
     & \left\|\mathbf{M}\right\|^2_F= \sum_{s=0}^{d-1}|R_s|\frac{cos^2(2\pi sx)}{|R_s|^2}\leq \sum_{s=0}^{d-1} \frac{1}{|R_s|}=\Delta(R) \quad \text{independent of $x$} \\
     & \left\|\mathbf{M}'_R \right\|_F \leq \left\|\bSigma_R \right\|_2\|\mathbf{M}'_R\|_F \quad \|\mathbf{M}'_R\|_2 \leq \|\bSigma_R\|_2\|\mathbf{M}'_R\|_2
 \end{align*}
 Then using Hensen-Wright inequality Lemma~\ref{lem:hens} we get 
 \begin{align*}
     &Pr \left[ \left|Tr(\mathbf{M}'_R)- \frac{1}{n}\sum_{l=1}^m {\y^{(l)}}^T \mathbf{M}'_R \y^{(l)} \right| > \epsilon\|\bSigma\|_2 \right] \\
     & \leq 2\exp \left(-cn \, \min \left(\frac{\epsilon^2\|\bSigma\|_2^2}{\|\mathbf{M}'_R\|_2^2}, \frac{\epsilon\|\bSigma\|_2}{\|\mathbf{M}'_R\|_2} \right)  \right)\\
     & \leq 2\exp\left(-cn \min \left(\frac{\epsilon^2}{\|\mathbf{M}_R\|_F^2}\frac{\|\bSigma\|_2^2}{\|\bSigma_R\|_2^2}, \frac{\|\bSigma\|_2}{\|\bSigma_R\|_2}\frac{\epsilon}{\|\mathbf{M}_R\|_2}\right) \right)\\
     & \leq 2 \exp(-cn\kappa)
     \end{align*}
    Finally  we bound the error as follows 
\begin{align*}
Pr\left[ |L_e(x)|\geq \epsilon\|\bSigma\|_2 \right]&  \leq 2 \exp(-cn\kappa)    
 \end{align*}
where $\kappa = \min(1, \frac{\epsilon^2\|\bSigma\|_2^2}{\Delta(R)\|\bSigma_R\|_2^2})$

Using union bound on the $2d $ different values of $x$ we get  $\|\bSigma-\Tilde{\bSigma}\|_2 \leq \epsilon \|\bSigma\|_2$ with probability $1- 4d\exp(-cn\kappa)$. The number of sample is $n= \frac{1}{c\kappa}\log (\frac{d}{\delta})$.

\end{proof}

\begin{remark}
Compared to the bound $n= O(\frac{log(d/\epsilon\delta)}{\kappa})$ in \cite{toep}, we improved the bound to $n= O(\frac{log(d/\delta)}{\kappa})$. The improvement is small but in terms of proof technique it has significance. Due to the circulant embedding of the Toeplitz matrix, we manage to bound the error $\left\| \bSigma- \Tilde{\bSigma}\right\|$ by taking maximum over only $2d $ different frequency where as previously the bound was on continuous range of frequency. \cite{toep} uses $\epsilon$-net type argument to bound the error over all frequencies in the domain which leads to the $\epsilon$ factor in the logarithm term in the sample complexity. 
\end{remark}

==> relt.tex <==
\section{Related work}
\begin{comment}
\Cam{
A dump of references to papers that use shortest path based covariance matrices. Should be helpful in writing intro:
\begin{itemize}
    \item SPATIAL MODELLING IN IRREGULARLY SHAPED
REGIONS: KRIGING ESTUARIES. Rathbun.
\item Kriging in estuaries: as the crow flies, or as the fish swims?
\item \url{https://link.springer.com/article/10.1007/s00477-011-0483-7}
\item Predicting stream temperatures: geostatistical
model comparison using alternative distance
metrics.
\item Estimating covariance in terms of shortest path distance in ecology:\\
https://www.ncbi.nlm.nih.gov/pubmed/15315694\\
\item https://link.springer.com/content/pdf/10.1023/A:1024409116214.pdf
\end{itemize}
}
\end{comment}
The problem of covariance estimation with access to all the entries of the sample data is a classical problem and has been studied extensively in \cite{kay1981spectrum,burg1982estimation,barton1997structured}. Estimation of covariance matrix with sparse ruler  has been studied in \cite{toep,lawrence2019low}. The graph dependent covariance structure 


Shortest distance based \cite{arnaud2003metapopulation,kurtz2015sparse,gardner2003predicting,boisvert2011modeling,little1997kriging,rathbun1998spatial}

The 
